Dance Style Transfer with Cross-modal Transformer

We present CycleDance, a dance style transfer system to transform an existing motion clip in one dance style to a motion clip in another dance style while attempting to preserve motion context of the dance. Our method extends an existing CycleGAN architecture for modeling audio sequences and integrates multimodal transformer encoders to account for music context. We adopt sequence length-based curriculum learning to stabilize training. Our approach captures rich and long-term intra-relations between motion frames, which is a common challenge in motion transfer and synthesis work. We further introduce new metrics for gauging transfer strength and content preservation in the context of dance movements. We perform an extensive ablation study as well as a human study including 30 participants with 5 or more years of dance experience. The results demonstrate that CycleDance generates realistic movements with the target style, significantly outperforming the baseline CycleGAN on naturalness, transfer strength, and content preservation.

==> Images/o.tex <==
% \begin{table}[]
% \caption{\textbf{Quantitative objective evaluation: }Motion Fréchet distance (MFD) and pose Fréchet distance (PFD) for the five competing models, includes the baseline model, our proposed CycleDance, as well as the ablations. 
% BJ2LC denotes transferring from ballet-jazz to locking dance. Correspondingly, LC2BJ denotes transferring from locking dance to ballet-jazz.
% }


% \resizebox{\columnwidth}{!}{
% \begin{tabular}{ccccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{MFD}      & \multicolumn{2}{c}{PFD}    \\
%                       & BJ2LC           & LC2BJ           & BJ2LC           & LC2BJ           \\
% \midrule
% CycleGAN-VC2           & 9.9430          & 3.4063.         & 0.4897          & 0.3499           \\
% CycleTransGAN          & 3.5643          & 0.7886          & 0.4749          & 0.2501          \\
% CycleTransGAN+CL       & 2.9188          & 0.5848          & 0.4897          & 0.2543          \\
% CycleCrossTransGAN     & 2.7446          & 0.5819          & 0.4419          & 0.2244          \\
% \textbf{CycleDance}    & \textbf{2.6109} & \textbf{0.5755} & \textbf{0.4216} & \textbf{0.2230} \\
% \bottomrule
% \end{tabular}
% }

% \label{tab:obj}
% \end{table}

% table 2
% \begin{table*}[]
% \centering

% \caption{\textbf{Quantitative objective evaluation: } Motion Fréchet distance (MFD) and pose Fréchet distance (PFD) for the five competing models, among the waacking, house, hip-hop, pop, locking, and ballet-jazz dance. 
% }

% \resizebox{0.7\columnwidth}{!}{
% \begin{tabular}{ccc}
% \toprule
% Method              & MFD                  & PFD                   \\ \midrule
% CycleGAN-VC2        & 3.3808          & 0.4565          \\
% CycleTransGAN       & 1.5737          & 0.4017          \\
% CycleTransGAN+CL    & 1.4350          & 0.3879          \\
% CycleCrossTransGAN  & 1.3904          & 0.3667          \\
% \textbf{CycleDance} & \textbf{1.3070} & \textbf{0.3612} \\ \bottomrule
% \end{tabular}
% }
% \label{tab:obj_2}

% \end{table*}


==> introduction.tex <==
\section{Introduction}

% 1. significance: why should one care?
% Transferring styles of various multimedia, such as images \cite{gatys2016image}, music \cite{brunner2018symbolic} and animation of human locomotion \cite{mason2022real}, has become commonplace thanks to recent advancements of deep neural networks. Transferring human movement styles has many applications in computer graphics, such as changing the gait of a video game character or conveying the personalities of different characters. 
Style transfer methods facilitate art creation of a target style for media such as images \cite{gatys2016image} and music \cite{brunner2018symbolic}. Similar methods are promising for creators to use an existing dance sequence as a starting point to generate variations across different movement styles. In a video game context, these style variations may -e.g.~be associated to different characters with different attributes or personalities. In a choreographic context, such a tool may lead to hybrid human-artificial creative processes, where style transfers are used to iterate on interesting, unexpected, or complementary variations of an initial choreographic material. 
% 2. status quo: what has already been done?
% Style transfer for sequential data in earlier research tends to require parallel data that assume a direct correspondence between instances in different styles or domains \cite{robinson2019sequence}. To address this limitation, cycle-consistent adversarial networks (CycleGAN) \cite{zhu2017unpaired}, adaptive instance normalization (AdaIN) \cite{karras2019style}, etc., were introduced. These works were successful in handling simple locomotive or exercise motions~\cite{mason2018few,du2019stylistic,aberman2020unpaired} and domain transfers between adults and children. 

Existing research on transferring human movement styles largely focuses on simple locomotive or exercise motions~\cite{mason2018few,du2019stylistic,aberman2020unpaired} and domain transfers between adults and children. Technical methods for transferring such sequential data include cycle-consistent adversarial networks (CycleGAN) \cite{zhu2017unpaired} and adaptive instance normalization (AdaIN) \cite{karras2019style}.
% 3. research gap: what is missing?
However, a research gap remains for applying similar techniques to enable style transfer of more complex movements, such as dance movements. Dance movements usually have no explicit functional purpose and tend to exhibit considerable richness in posture, rhythm and their composition. Generation of dance movements can be particularly challenging since it demands a multi-layer approach that captures motion qualities such as the coordination of joint dynamics and socio-cultural factors associated with the production and perception of the movement. Meanwhile, there exist a variety of such characteristics within different dance styles, originating from different historical backgrounds. Dance styles could be thought more generally of as styles of performing certain dance movements rather than strictly dance genres. This adds another layer of complexity to the generation of high-quality dance movements of a specific target style. 
All these challenges call for computational models that can capture both high-frequency features and long-term dependencies over time, and as such generate realistic dance with aesthetic and coherence.


% A model is desired for capturing both high-frequency features and long-term dependencies over time, and as such generating realistic dance with aesthetic and coherence. This motivates us to provide a novel tool for dance style transfer. Computational models that overcome this level of complexity can unlock many potential applications, such as tool development for complex motion design in choreography, gaming, and animation, which can offer artistic and scientific innovations to the field of dance. 
% % music
Moreover, dance is commonly accompanied by music which can provide tremendous clues for understanding and composing movement. Recent works have shown the effectiveness of music-conditioned dance synthesis~\cite{valle2021transflower, chen2021choreomaster}, which can directly generate dance motion given music context. However, it is unclear whether music context will also facilitate style transfer tasks and how such a multi-modal input should be processed in this context. 

% 4. filling the gap: how are you addressing this gap? 
% method
In this paper, we propose CycleDance, a multimodal system (see Figure \ref{fig:teaser}) for dance style transfer. CycleDance adopts a generative scheme by extending CycleGAN-VC2 \cite{kaneko2019cyclegan} to work with unpaired data. To tackle the challenges identified above, we exploit a cross-modal transformer architecture \cite{valle2021transflower} that aims to effectively capture relevant features among different modalities so as to enhance style transfer quality. Specifically, we design a two pathways transformer-based architecture to extract temporally aligned motion and music representations in the context of style transfer. We further propose to train CycleDance progressively with a curriculum learning scheme inspired by Fu et al. \cite{fu2021cycletransgan}. This alleviates issues of instability in training large adversarial models and premature convergence that can lead to inferior performance. 
% evaluation
We evaluate our framework on the AIST++ \cite{tsuchida2019aist} dance database, with the analysis focused on transfer between various dance genres.
Two new metrics based on probabilistic divergence and selected key pose frames are proposed to quantitatively assess the quality of dance style transfer. Moreoever, we invite a group of human participants with extensive dancing experience to provide a subjective evaluation and insights from an expert perspective. These evaluations show that CycleDance greatly outperforms a baseline method and its ablative versions.
% demo
As an illustration, a video with generated examples can be found at \href{https://youtu.be/kP4DBp8OUCk}{ https://youtu.be/kP4DBp8OUCk}. 

% 5. impact: what does this unlock in terms of potential uses or applications?
% While existing generative models offer limited user control over the type of output they create \cite{guo2020action2motion, petrovich2021action}, our approach enables creators to use an existing dance sequence as a starting point to potentially create variations of the same motion across different movement styles. In a video game context, these style variations may -e.g.~be associated to different characters with different attributes or personalities. In a choreographic context, such a tool may lead to hybrid human-artificial creative processes, where style transfers are used to iterate on interesting, unexpected, or complementary variations of an initial choreographic material. 

% 6. contributions
In summary, our contributions are mainly as follows:
\begin{itemize}
\item Our approach is, to the best of our knowledge, the first to combine complex dance motion and music context in the style transfer task, 
% We develop a cross-domain CycleGAN-based model with transformer encoders to extract rich motion and music context features for effective style transfer. Curriculum learning is further introduced to tackle technical difficulties stemming from training large adversarial models. 
% More importantly, 
%Compared to earlier style transfer work, we consider more complex dance movements that go beyond simple locomotion or exercise motions, 
unlocking potential applications
%, such as tool development for complex motion design 
in choreography, gaming, and animation, as well as in tool development for artistic and scientific innovations in the field of dance. 
\item We introduce new metrics based on probabilistic divergence and selected key pose frames for gauging transfer strength and content preservation in the context of dance movements. 
\item We provide an extensive user study of the proposed model. The evaluations and insights from a group of experienced dance performers reveal essential aspects of designing such systems.
\end{itemize}

% 7. paper outline
% The paper proceeds as follows:
% Section \ref{sec:related} gives an introduction to previous works on the topic of dance style transfer, including style transfer, motion style transfer, and music-conditioned motion synthesis. 
% Section \ref{sec:method} formulates the problem and describes the full design of our proposed framework for dance style transfer. 
% Section \ref{sec:exp} presents the experimental setup and discusses results, compares the results to the baseline. 
% Finally, Section \ref{sec:conclusion} outlines a plan for future work and concludes the paper. 

